Programmable Agents

We build deep RL agents that execute declarative programs expressed in formal language. The agents learn to ground the terms in this language in their environment, and can generalize their behavior at test time to execute new programs that refer to objects that were not referenced during training. The agents develop disentangled interpretable representations that allow them to generalize to a wide variety of zero-shot semantic tasks.

==> 100-canonical-failure.tex <==
\section{Why do standard networks fail to generalize?}

\begin{figure}
    \centering
    \includegraphics[width=0.15\linewidth]{artwork/canonical-actor}
    \quad
    \includegraphics[width=0.15\linewidth]{artwork/canonical-critic}
    \qquad\qquad
    \includegraphics[width=0.425\linewidth]{artwork/reasoning-diagram}
    \caption{\textbf{Left:} Structure of the canonical actor and critic networks. Arrows represent linear layers; $\tanh$ activations are used throughout both networks. \textbf{Right:}  Two possible reasoning strategies for canonical networks on the programmable reaching tasks.  The top row shows a generalizable strategy where the components of the task each index properties of the objects, and a second reasoning step derives the target position index from the coincidence of property indices.  The bottom row shows a degenerate strategy where the task representation directly indexes the target position.  This strategy cannot generalize to novel combinations of properties because the mapping from target properties to the index of the target position is arbitrary.}
    \label{fig:canonical-networks}
\end{figure}

Why do standard deep architectures fail to generalize on our tasks?  Recall that the experiment in Section~\ref{sec:standard-failure} shows that the canonical architecture is able to perform quite well in the 2-C condition where it sees all tasks at training time.  Why then does it fail in the held out condition of the 2-L design?  Generalization to new target locations is known to work quite well~\cite{lillicrap2015continuous}; how is generalization to a new target object different?

In this section we provide a possible answer to these questions by examining the type of reasoning strategy that generalization in the 2-L setting requires.  We consider two degenerate reasoning strategies, either of which are sufficient to explain the failure of the canonical architecture on the held out task in 2-L.  We argue that success in the training conditions does not require agents to distinguish between these three approaches, and absent any externally imposed inductive bias it is natural to expect them to settle on one of the simpler, degenerate strategies.

\subsection{Three reasoning strategies}

Consider the structure of the observation vector for the canonical network in a 2x2 design.  The following diagram shows a schematic representation of the contents of the observation.
\begin{center}
\includegraphics[width=0.425\linewidth]{artwork/canonical-features}
\end{center}
The observation contains joint angles for the arm, a group of features for each object, and some features describing the task, which in our case is always a combination of a color and a shape.  Each object has some features describing its location (and orientation) as well as some features describing its properties.

Objects locations are represented in the coordinate frame of the hand, so if the index of the target location in the features is known then the task becomes to make the features at that index zero (or as near to zero as possible).  There are four objects, and thus four possible target indexes, and the task specifies which feature index the network should attempt to minimize.

A generalizable reasoning strategy that achieves this is as follows:
\begin{center}
\includegraphics[width=0.425\linewidth]{artwork/generalizable-reasoning}
\end{center}
The task has two components, a color and a shape, and each component refers to two properties at two different indexes.  There is one index where both references agree, and the target location occurs at a fixed offset from that index. 

==> 120-videos.tex <==
\section{Videos}
\label{sec:videos}

Videos of an agent completing zero shot tasks under different conditions.  See Section~\ref{sec:generalization} for a description of each condition.

\begin{center}
\begin{tabular}{l|l}
\textbf{Condition}  & \textbf{Video} \\
\hline
~&~\\
train               & \hideurl{} \\
eval                & \hideurl{} \\
only color          & \hideurl{} \\
only shape          & \hideurl{} \\
three blocks        & \hideurl{} \\
five blocks         & \hideurl{} \\
nine blocks         & \hideurl{} \\
not color           & \hideurl{} \\
not shape           & \hideurl{} \\
ignore new blocks   & \hideurl{} \\
new shape           & \hideurl{} \\
new color           & \hideurl{} \\
new shape new color & \hideurl{}
\end{tabular}
\end{center}
